Spotr: GPS Spoofing Detection via Device Fingerprinting

As the worlds predominant navigation system GPS is critical to modern life, finding applications in diverse areas like information security, healthcare, marketing, and power and water grid management. Unfortunately this diversification has only served to underscore the insecurity of GPS and the critical need to harden this system against manipulation and exploitation. A wide variety of attacks against GPS have already been documented, both in academia and industry. Several defenses have been proposed to combat these attacks, but they are ultimately insufficient due to scope, expense, complexity, or robustness. With this in mind, we present our own solution: fingerprinting of GPS satellites. We assert that it is possible to create signatures, or fingerprints, of the satellites (more specifically their transmissions) that allow one to determine nearly instantly whether a received GPS transmission is authentic or not. Furthermore, in this paper we demonstrate that this solution detects all known spoofing attacks, that it does so while being fast, cheap, and simpler than previous solutions, and that it is highly robust with respect to environmental factors.

==> background.tex <==

\section{Background Information}
\label{sec::background}
In this section we discuss central concepts necessary to understand 
\cite{keysightGNSSapplicationnote}

\subsection{GPS Satellite System}

\label{sec::GPSsystem}
The \textit{Global Positioning System} (GPS) is the more robust and fully-featured successor to \textit{Transit}, the original Global Navigation Satellite System (GNSS).  GPS is built upon three components:  the ground stations (\textit{control segment}), the satellites (\textit{space segment}), and the navigator (\textit{user segment}).  The ground stations are administrative in nature, mostly used for monitoring satellite health, performing military functions (command \& control, etc.), and for ensuring that the satellites remain in a formation called a \textit{constellation}.  This formation ensures that users have access to position, velocity, and time information all over the globe.
\subsection{Digital Receiver}
Fig.~\ref{fig::receiver} illustrates a block diagram of GPS receiver. The main components of GPS receiver are (i) RF front-end, (ii) acquisition module and (iii) tracking module and (iv) Position, Velocity, Time (PVT) estimator module. The RF front-end investigates if satellite signals are available. The acquisition module searches for the delayed versions of any PRN's reference signal after estimating the Doppler shift and compensating for it. The role of a Tracking block is to follow the evolution of the signal synchronization parameters: code phase, Doppler shift and carrier phase. The PVT estimator uses the information collected from satellites to report a PVT solution. The most common method to do so is called multilaterization. The idea behind multilaterization is that an accurate estimate of longitude, latitude and elevation of a GPS signal requires data collected from at least four satellites. This can be used for solving a localization problem with three unknown parameters. 


\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figs/GPS_receiver.pdf}
    \caption{Block diagram of GPS digital receiver.}
    \label{fig::receiver}
\end{figure}

For a more thorough review of GPS, its applications, and its vulnerabilities, there are a number of available resources including \cite{U.S.A.F.GPS:System, 2017UnderstandingApplications,Groves2013PrinciplesSystems,2015GNSSCountermeasures,Wu2018AdaptiveGNSS}. 






==> tabs/data_list.tex <==
\small
\begin{tabular}{c|c|c|c|c|c|c|c}
\hline
\textbf{Dataset}        & \textbf{collection date} & \textbf{spoofing type} & \textbf{spoofing power status} & \textbf{ multipath } & \textbf{duration} & \textbf{start time} & \textbf{location} \\ \hline \hline

\textbf{TexBat:clean}     & July 2015                & --                   & --                   & No      & 420 s   & --     & Texas         \\ \hline
\textbf{TexBat:clean}     & July 2015                & --                   & --                   & Yes     & 420 s   & --     & Texas         \\ \hline

\textbf{TexBat:ds1}     & Sep 2012                 & both                     & under-powered                    & No    & 420 s     & --     & Texas            \\ \hline
\textbf{TexBat:ds2}     & Sep 2012                 & time                   & over-powered           & No    & 420 s     & --     & Texas            \\ \hline
\textbf{TexBat:ds3}     & Sep 2012                 & time                   & matched-powered        & No    & 420 s     & --     & Texas            \\ \hline
\textbf{TexBat:ds4}     & Sep 2012                 & position               & matched-powered        & No    & 420 s     & --     & Texas            \\ \hline
\textbf{TexBat:ds5}     & Sep 2012                 & time                   & over-powered           & Yes   & 420 s     & --     & Texas            \\ \hline
\textbf{TexBat:ds6}     & Sep 2012                 & position               & matched-powered        & Yes   & 420 s     & --     & Texas            \\ \hline
\textbf{TexBat:ds7}     & July 2015                & time                   & matched-powered        & No    & 420 s     & --     & Texas            \\ \hline
\textbf{TexBat:ds8}     & July 2015                & time                   & matched-powered        & No    & 420 s     & --     & Texas            \\ \hline

\textbf{VAclean}     & Sep 24, 2018              & --                   & --                       & No      & 60 min   & 4:10 pm   & \LocOne{}              \\ \hline
\textbf{VAclean}     & Sep 25, 2018              & --                   & --                       & No      & 60 min   & 4:10 pm   & \LocOne{}              \\ \hline
\textbf{VAclean}     & Sep 26, 2018              & --                   & --                       & No      & 60 min   & 4:10 pm   & \LocOne{}              \\ \hline
\textbf{VAclean}     & Sep 28, 2018              & --                   & --                       & No      & 60 min   & 4:10 pm   & \LocOne{}              \\ \hline

\textbf{NaiveAttacker} & Sep 24, 2018             & both                     & over-powered              & No     & 60 min    & --   & \LocOne{}               \\ \hline
\textbf{NaiveAttacker} & Sep 25, 2018             & both                     & over-powered              & No     & 60 min    & --   & \LocOne{}               \\ \hline
\textbf{NaiveAttacker} & Sep 26, 2018             & both                     & over-powered              & No     & 60 min    & --   & \LocOne{}              \\ \hline
\textbf{NaiveAttacker} & Sep 28, 2018             & both                     & over-powered              & No     & 60 min    & --   & \LocOne{}              \\ \hline

\textbf{VAclean}     & Dec 15, 2018                & --                   & --                     & No      & 60 min  & 12 pm     & Missouri             \\ \hline
\textbf{VAclean}     & Dec 15, 2018                & --                   & --                     & No      & 60 min  & 2 pm      & Missouri             \\ \hline
\textbf{VAclean}     & Dec 15, 2018                & --                   & --                     & No      & 60 min  & 8 pm      & Missouri             \\ \hline

\textbf{VAclean}     & Dec 16, 2018                & --                   & --                     & No         & 60 min   & 2 am     & Missouri             \\ \hline
\textbf{VAclean}     & Dec 16, 2018                & --                   & --                     & No         & 60 min   & 3:30 pm  & Missouri             \\ \hline
\textbf{VAclean}     & Dec 16, 2018                & --                   & --                     & No         & 60 min   & 7 pm     & Missouri             \\ \hline
\textbf{VAclean}     & Dec 16, 2018                & --                   & --                     & No         & 60 min   & 9 pm     & Missouri             \\ \hline
\textbf{VAclean}     & Dec 16, 2018                & --                   & --                     & No         & 60 min   & 11 pm    & Missouri             \\ \hline

\textbf{VAclean}     & Dec 17, 2018                & --                   & --                     & No      & 60 min     & 6 am   & Missouri             \\ \hline
\textbf{VAclean}     & Dec 17, 2018                & --                   & --                     & No      & 60 min     & 12 pm  & Missouri             \\ \hline
\textbf{VAclean}     & Dec 17, 2018                & --                   & --                     & No      & 60 min     & 10 pm  & Missouri             \\ \hline

\textbf{VAclean}     & Dec 18, 2018                & --                   & --                     & No      & 60 min   & 4 am    & Missouri             \\ \hline
\textbf{VAclean}     & Dec 18, 2018                & --                   & --                     & No      & 60 min   & 11 am   & Missouri             \\ \hline
\textbf{VAclean}     & Dec 18, 2018                & --                   & --                     & No      & 60 min   & 2 pm    & Missouri             \\ \hline
\textbf{VAclean}     & Dec 18, 2018                & --                   & --                     & No      & 60 min   & 11 pm   & Missouri             \\ \hline

\textbf{VAclean}     & Dec 19, 2018                & --                   & --                     & No     & 60 min   & 9 am   & Missouri             \\ \hline
\textbf{VAclean}     & Dec 20, 2018                & --                   & --                     & No     & 60 min   & 9 pm   & Missouri             \\ \hline
 
\textbf{NaiveAttacker} & Dec 15, 2018             & both                     & over-powered         & No      & 60 min   & 12 pm    & Missouri               \\ \hline
\textbf{NaiveAttacker} & Dec 16, 2018             & both                     & over-powered         & No      & 60 min   & 2 am    & Missouri               \\ \hline

\textbf{VAclean}     & Aug 23, 2019                & --                   & --                     & yes     & 10 min   & 4 pm     & \LocTwo{} (urban)            \\ \hline
\textbf{VAclean}     & Sep 10, 2019                & --                   & --                     & No      & 45 min   & 3 pm     & \LocTwo{} (football field)   \\ \hline
\textbf{VAclean}     & Nov 8, 2019                 & --                   & --                      & No      & 45 min   & 10 am    & \LocTwo{} (rooftop)             \\ \hline
\textbf{VAclean}     & Nov 8, 2019                 & --                   & --                      & No      & 50 min   & 11 am    & \LocTwo{} (rooftop)             \\ \hline

\textbf{SmartAttacker}   & Aug 23, 2019                & both               & adjusted-power          & No     & 10 min  & --  & \LocTwo{}              \\ \hline
\textbf{SmartAttacker}   & Sep 10, 2019                & both               & adjusted-power          & No     & 45 min  & --  & \LocTwo{}              \\ \hline

\textbf{SmartAttacker}   & Nov 8, 2019                & both               & adjusted-power           & No     & 50 min  & --  & \LocTwo{}              \\ \hline
\textbf{SmartAttacker}   & Nov 8, 2019                & both               & adjusted-power           & No     & 50 min  & --  & \LocTwo{}              \\ \hline

\end{tabular}
